Atmospheres of Brown Dwarfs

Brown Dwarfs are the coolest class of stellar objects known to date. Our present perception is that Brown Dwarfs follow the principles of star formation, and that Brown Dwarfs share many characteristics with planets. Being the darkest and lowest mass stars known makes Brown Dwarfs also the coolest stars known. This has profound implication for their spectral fingerprints. Brown Dwarfs cover a range of effective temperatures which cause brown dwarfs atmospheres to be a sequence that gradually changes from a M-dwarf-like spectrum into a planet-like spectrum. This further implies that below an effective temperature of < 2800K, clouds form already in atmospheres of objects marking the boundary between M-Dwarfs and brown dwarfs. Recent developments have sparked the interest in plasma processes in such very cool atmospheres: sporadic and quiescent radio emission has been observed in combination with decaying Xray-activity indicators across the fully convective boundary.

==> SarahC.tex <==

\section{Brown dwarf observations in different energy ranges}\label{s:obs}


\subsection{Optical and IR}
-- shortly introduce the different spectral types (late M, L, T, Y)
but mention that spectral types are confined to limited parts of
spectrum.  L dwarfs described and defined by \cite{martin99,
  kirkpatrick99, kirkpatrick05} and a spectral classification based on
molecular line strengths is mentioned. 
-- T dwarfs - \cite{geballe02} did the same.


There are $\sim$20 Y dwarfs known to date \citep{cushing11, luhman11,
  kirkpatrick12, kirkpatrick13, cushing14}. The majority of these have
spectral types ranging between Y0 and Y2 and were discovered using the
\textit{Wide-field Infrared Survey Explorer} (WISE). WISE was designed
to discover Y dwarfs, and the shortest wavelength band at 3.4$\mu$m
was selected to fall in the centre of the fundamental methane
absorption band at 3.3$\mu$m. The W2 filter at 4.6$\mu$m detects
radiation from the deeper, hotter layers in the brown dwarf
atmosphere. Combined, the W1-W2 colour is very red, allowing the
detection of Y dwarfs \citep{kirkpatrick11}. All the Y dwarfs show
deep H$_{2}$O and CH$_{4}$ absorption bands in their near-infrared
spectra, similar to late-T dwarfs. The $J$ band peaks of the Y dwarfs
are narrower than those of the latest type T dwarfs, and the ratio of
the $J$ and $H$ band flux is close to 1, effectively meaning that the
$J-H$ trend towards the blue for T dwarfs turns back towards the red
for Y0. This trend also occurs for the $Y-J$ colour.  It is though
this colour reversal is due to the alkali metals that dominate the
absorption in the shorter wavelengths being trapped in molecules, thus
reducing the opacity \citep{liu10}. While the $H$ band spectra of T
dwarfs are shaped by CH$_{4}$ and H$_{2}$O, for Y dwarfs as the
effective temperature decreases NH$_{3}$ absorption becomes important
\citep{lodders02, burrows03}. \citet{cushing11} estimate the effective
temperatures of the Y0 dwarfs are between 350 and 500 K, with masses
between $\sim$5 and 20 M$_{\rm Jup}$.  However, using a luminosity
measurement derived using a $\Spitzer$ based parallax, \citet{dupuy13}
estimate their effective temperatures to be typically 60-90 K
hotter. The difference in temperatures is possibly related to the fact
that in the near-IR, where the spectra are obtained, only 5\% of the Y
dwarf flux is emitted and the models do not always accurately
reproduce the observed spectra \citep{dupuy13}. Using more advanced
non-equilibrium models containing sulphide and chloride clouds
\citep{allard10, morley12}.  \citet{beichman14} do obtain the lower
effective temperatures, claiming that the \citet{dupuy13} result
depends on a model dependent bolometric correction, which also is also
quite uncertain. \citet{dupuy13} also highlight the WD0806-661B as
being the most likely candidate for lowest mass, and lowest
temperature Y dwarf at 6-10 M$_{\rm Jup}$ and 330-375 K. As
WD0806-661B is in a wide binary with a DQ white dwarf \cite{luhman12,
  luhman11}, it has a well defined age derived from the cooling age of
the white dwarf and it's main sequence lifetime derived using an
initial mass-final mass relation \citep{casewell09, dobbie09}.

\subsubsection{Metallicity}
Low metallicity brown dwarfs (subdwarfs) provide an insight into the coolest, old brown dwarfs. Not only from a formation point of view, proving that low metallicity clouds can form substellar objects, but also for comparison to low metallicity extrasolar planets. 

There are, however, only a handful of ultracool subdwarfs known to date \citep{burgasser03, burgasser04, cushing09, sivarani09, lodieu10, kirkpatrick10, lodieu12, mace13, kirkpatrick14}, and even fewer ($\sim$10) that are L dwarfs. Indeed, of the 29 objects known to date, only  6 have spectral type later than L2 \citep{kirkpatrick14}. Many of these objects have been identified as potential members of the Galactic Halo. \citet{burgasser08} noted that L subdwarfs are overluminous in $M_{J}$, but this changes to slightly underluminous by $M_{K}$. This change is 
attributed to a reduced condensate opacity causing strong TiO, FeH, Ca $\sc{I}$ and Ti $\sc{I}$ features, and enhanced
collisional-induced H$_{2}$ opacity in the $K$ band \citep{ackerman01, tsuji96, burgasser03, burgasser07}. This effect also causes red colours in the optical wavelengths and bluer colours than L dwarfs of the same spectral type.  The naming scheme for subdwarfs follows that for M dwarfs developed by \citet{gizis97} and upgraded by \citep{lepine}, moving from dM for metal rich M dwarfs to subdwarfs (sdM), extreme subdwarfs (esdM) and ultra subdwarfs (usdM) in order of decreasing metallicity.
There has been a suggestion by \cite{kirkpatrick14} that there is an L subdwarf "gap" between the early L and late L subdwarfs caused because lower metallicity generally corresponds to older objects. Thus at older ages there is a gap in temperature between the the hottest members of the population, and the coolest, lowest mass members of similarly aged hydrogen burning stars. This temperature gap is predicted to increase with older populations. This can be seen in Figure 29 of \citet{kirkpatrick14}.

Recently, a population of T subdwarfs has emerged \citep{burningham14, mace13}. T dwarfs in are very sensitive to small changes in metallicity - a low metallicity T dwarf with a shift of 0.3 dex can change the $H-$[4.5] colours of T8 dwarfs as much as a 100K change in effective temperature \citep{burningham13}. The T dwarfs exhibit enhanced $Y$ and depressed $K$ band flux indicative of a high gravity and low metallicity atmosphere \citep{burgasser02}. The increased $Y$ band is caused as the lower metallicity means a reduced opacity in the wings of the alkali lines, resulting in a brighter and broader peak flux \citep{burgasser06}.  The $K$ band flux depression is caused by pressure-enhanced collision induced absorption by molecular hydrogen (CIA H$_{2}$; \citealt{saumon94}). 

\subsubsection{Gravity}

Young, low gravity brown dwarfs have very similar properties to directly-imaged exoplanets \citep{fah2013}. 
It has been suggested that younger brown dwarfs may have thick clouds in their atmospheres that are not 
present in older objects of the same temperature \citep{barman11, currie11, madhusudhan11}. 

There are many brown dwarfs that have been identified in open star clusters such as those in Sigma Ori \cite{bihain09, pena12} , Serpens \cite{spezzi12} or the Pleiades \cite{casewell11, casewell07}. However,  there also exists a field population of low gravity, young brown dwarfs \citep{reid08, cruz09, kirkpatrick10}.  A comprehensive scheme for  defining the gravity of these objects was devised by \citet{kirkpatrick08} and \citet{cruz09} in the optical, and \citet{allers13a, allers13b} in the near-infrared. The classification relies on a suffix of $\alpha$, $\beta$, or $\gamma$ to be added to the object's spectral type, to indicate the gravity. $\alpha$ implies a normal gravity field dwarf (age $\sim$ 1Gyr), whereas $\beta$ is an intermediate-gravity object of $\sim$100 Myr, and $\gamma$ represents an age of $\sim$10-30 Myr. 
In the optical wavebands the suffixes are assigned based on measurements of the Na $\sc{I}$ doublets and the K $\sc{I}$ doublets which are weaker and sharper in a low gravity object, the VO absorption bands which are stronger than for a high gravity dwarf, and the FeH absorption features which are weaker in low gravity.  In the near-infrared, 
the depth of the VO and FeH bands are considered as well as the alkali lines. The shape of the $H$-band is also taken into consideration as a more peaky, triangular H band, caused by steam absorption is a sign of low gravity \citep{lucas01, rice11}. All of these features are altered as there is less pressure broadening due to the object having a low surface gravity \citep{rice11, allers13a}.
In general, alkali absorption features are weaker, and the overall colours of lower gravity objects are redder than those of their higher gravity counterparts, by as much as 0.8 mag in $J-K_{s}$ and 0.25 mag redder in $W1-W2$ \citep{faherty13}. The redder colour is due in part to the changes in the near-infrared broadband features, but also due to more photospheric dust. (FIND A REFRERNCE) An additional feature is that while young M dwarfs are brighter than their older counterparts, young L dwarfs are underluminous in the near-infrared for their spectral type. This may be due to the additional dust in their photosphere \citep{faherty13a} or due to a cooler spectral type/temperature relation being required.

It is possible that many of these low gravity field brown dwarfs may belong to moving groups. There have been many kinematic measurements of brown dwarfs (e.g. \citealt{schmidt07, faherty09, faherty11, faherty12, faherty13a, dupuy13, marocco13}, identifying moving group members \cite{Jameson08, Casewell08} of which the majority concentrate on  young moving groups such as AB Doradus, $\Beta$ Pictorus, and Tucana-Horologium \citep{kirkpatrick06, kirkpatrick10, cruz09, allers10, rice10}.

There are two directly-imaged planetary mass companions that have estimated effective temperatures in the brown dwarf regime. 2M1207b ($\sim$ 10 Myr, $\sim$ 1100 K, Spt$\sim$mid L) and HR8799b ($\sim$30 Myr, $\sim$1600 K, Spt$\sim$ early T). These planets are underluminous and have unusually red near-infrared colours, as well as displaying the characteristic peaked $H$-band spectra. There are 30 brown dwarfs that have been kinematically lined to moving groups and association aged between 10 and 150 Myr, that share these features, thus indicating that low gravity brown dwarfs may provide a clue as to the atmospheric processes occurring on young exoplanets.

\subsection{X-ray and UV observations}

There have been numerous searches for X-ray detections of brown dwarfs due to their indicator of magnetic activity. However, it is clear that after the spectral type M7-M8, there is a decline in emission, consistent with the decline seen in chromospheric H$\alpha$ emission \citep{gizis00, mohanty03, west04}.   The relationship normally used to describe this relates X-ray activity ($L_{X}/L_{bol}$)  and rotation, and there is a similar relation for H$\alpha$.   There is also a relationship between the radio (L$_{v,R}$) and X-ray luminosities which is linear for active F-M stars and L$_{X} \propto$ L$_{v,R}^{\alpha}$ where $\alpha$$\sim$0.73. . This is known as the G"/{u}del-Benz relation \citep{gudel93, benz94}. There have been many searches \citep{stelzer03, berger05, stelzer06} for X-ray emission in L dwarfs, however, only one detection to date \citep{audard07},  the L dwarf binary Kelu-1 that was detected with $Chandra$ in the energy range of 0.63, 0.86, 1.19 and 1.38 keV, resulting in an estimation of the  0.1-10 keV X-ray luminosity to be $L_{X}=2.9\times10^{25}$ erg s$^{-1}$. It is suggested that this emission does not originate from flares, and indeed there was no concurrent radio detection at a frequency $\sim$8 GHz \citep{audard07}.
\citep{audard07} suggested that the ratio between luminosity and bolometric luminosity increase with decreasing effective temperature, which dominates the bolometric luminosity, in the radio. However in the X-rays, the ratio decreases with effective temperature, as does the similar relation for H$\alpha$.  Their conclusions were that the chromospheric magnetic activity (H$\alpha$ emission) and the activity in the hot coronal loops (X-ray emission) decreases with effective temperature, indicating a different mechanism responsible for the radio emission in ultra cool dwarfs.

 \citet{williams13c} suggest that ultracool dwarfs with strong axisymmetric magnetic fields tend to have $L_{v,R}/L_{X}$ consistent with the G\"{u}del-Benz relation,  while dwarfs with weak non-axisymmetric fields are radio luminous. Slower rotating dwarfs have strong convective field dynamos and so also stay near the G\"{u}del-Benz relation, whereas rapid rotators may have dynamos in either mode so some violate the G\"{u}del-Benz relation, and some do not.  \citet{williams13c} also note that weaker field dwarfs tend to have later spectral types, and lower X-ray luminosity, which may be related to their cooler temperatures. They also note that in general, radio-bright sources, tend to be X-ray under luminous compared to the radio dim sources.

There are no detections of brown dwarfs  emission in the UV known to result from atmospheric processes. However, brown dwarfs with disks such as the young TW Hydra member 2MASS1207334-393254 have been observed in the UV. H$_{2}$ fluorescence is detected and attributed to accretion \citep{gizis05}. As such, this mechanism is beyond the scope of this review.

\subsection{H$\alpha$}

The strength of H$\alpha$ emission in late M and L dwarfs also decreases with lower mass and later spectral type. \citet{schmidt07} estimate that of their 152 strong 
sample, 95\% of M7 dwarfs show H$\alpha$ emission (which is consistent with \citealt{gizis00}) which declines with spectral type to 8\% of L2-L8 dwarfs showing H$\alpha$. For the L dwarfs in particular, 50\% of L0 dwarfs 
being active declines to  20-40\% of L1 dwarfs and only 10\% of L2 dwarfs and later spectral types. This decline is similar to the breakdown in rotation-activity relationship seen for the X-ray activity. This decline in H$\alpha$ has been attributed to the high electrical resistivities in the cool, neutral atmospheres of these dwarfs \citep{mohanty02}, although no firm conclusions have been made.

Despite this decline, some objects of late spectral type do show H$\alpha$ emission. The L5 dwarfs 2MASSJ01443536-0716142 and  2MASS1315-26 have shown H$\alpha$ emission.
For 2MASSJ1044-0716, this emission declined over time and was not detected in subsequent spectra obtained a year later \citep{liebert03}. This flaring has been detected in other ultracool dwarfs such as BRI0021-0214 \citep{reid99}. 2MASS1315-26 is a high proper motion source that has pronounced and sustained H$\alpha$ emission \citep{hall02, gizis02, burgasser11}. The kinematics suggest that this source is not young (age $\sim$ few Gyr), meaning it is likely 
just above the hydrogen mass burning limit. \citep{burgasser13}.
In quiescence, these objects show H$\alpha$ fluxes similar to those of other dwarfs of the same spectral type. However in outburst, 2MASS0144-0716 has an H$\alpha$ flux measurement more than 10 times higher than the mean \citep{liebert03}, and for 2MASS1315-26 the optical emission is $\sim$ 100 times stronger than for L dwarfs of a similar spectral type \citep{hall02}.


\subsection{Radio emission}

In cool stars, the magnetic dynamo mechanism is used to explain
magnetic field generation in solar-type stars, and there is a direct
correlation between rotation and magnetic activity indicated by
H$\alpha$, X-rays and radio emission \citep{noyes84, stewart88,
  james00, delfosse98, pizzolato03, browning10, reiners09,
  morin10}. As this dynamo operates at the transition layer between
the radiative and convective zones, the mechanism cannot explain radio
activity in fully convective dwarfs ($>$M3).  As already discussed,
H$\alpha$ and X-ray activity does, however continue into the late M
dwarf regime, but the tight correlation between X-ray and radio
luminosity breaks down (G{\"u}del-Benz relation: \citealt{gudel93,
  benz94}) suggesting a separate mechanism is responsible for this
emission.

A number ($\sim$10 \% reference) of brown dwarfs have been detected to
be radio loud.  This non-thermal emission may be low level quiescent
\citep{berger02}, exhibiting variability \citep{antonova07}, showing
variability that is periodic and linked to rotation \citep{berger05,
  mclean11}, highly polarised and bursting \citep{burgasser05},
pulsing synchronised with the rotation period and highly polarised
\citep{hallinan07, berger09} or a combination of some of these
\citep{williams13b}.


Some of these objects (TVLM513-46546, 2MASSJ0036+1821104, LSRJ1835+3259, 2MASSJ1047539+212432 \citealt{rw12, hallinan08}) emit periodic, 100\% polarised radiation, normally detected at 4-8 GHz with spectral luminosities of $\approx
10^{13.5}$~\ergshz e.g.\cite{had+06,rw12}.
These pulses have been confirmed to be caused by the cyclotron maser instability (CMI), the emission mechanism that occurs on Jupiter \citep{t06, nbc+12, mmk+12}.  CMI emission requires a relatively tenuous population of
energetic particles confined to a relatively strong magnetic field; in
particular, one must have $f_\text{ce} \gg f_\text{pe}$, where $f_\text{ce} =
e B / m_e c$ is the cyclotron frequency and $f_\text{pe} = \sqrt{4 \pi e^2 n_e
  / m_e}$ is the plasma frequency. Whenever detailed observations are
available, the necessary free energy in the plasma is seen to be provided by
field-aligned electric currents, which can originate in
magnetospheric-ionospheric (M-I) shearing and possibly plasma instabilities. 
These observations imply that BDs can
self-generate stable, $\sim$kG-strength magnetic fields \citep{b06b}. 

Although this mechanism for emission is quite well characterised, and can account for the polarised flaring behaviour, two of these dwarfs also produce quiescent, moderately polarised emission. This indicates that a second mechanism such as synchrotron or gyrosynchrotron emission \citep{berger02, osten06, ravi11} may be occurring, or that the CMI emission is becoming depolarised in some way as it crosses the dwarf's magnetosphere. It has been suggested that some of the variability seen in these sources may be due to variation in the local plasma conditions, perhaps linked to magnetic reconnection events \citep{schmidt07} or due to other charged events in the plasma (IS THIS REASONABLE? CAN I CITE CRAIG AND PAUL HERE???)
Additionally, there are some radio active ultracool dwarfs  that exhibit behaviour that is not due to CMI (e.g. 2MASS13153094-2649513AB \citealt{burg2013} - which also displays H$\alpha$ emission). This particular source emits strong quiescent emission, with peak fluxes comparable to the fluxes detected for other ultracool dwarfs while in outburst.

 It is also still unknown what features distinguish radio "active" from radio "inactive" dwarfs. The relationship may depend on mass, effective temperature, activity, magnetic field strength and rotation rate. All the known radio "active" dwarfs have a high $V$ sin $i$ value, indicating short rotation periods ($\sim$3hrs) \citep{antonova13, williams13a}. This may indicate a link between rotation rate and emission, but could also indicate the dependence is not on the velocity but on the inclination angle, $i$, thus making detection of radio emission dependent on the line of sight and the radiation emitted beamed \citep{hallinan08}.
 

\subsection{Observed variability in Brown Dwarfs}\label{ss:obsvariab}

As the number of brown dwarfs has increased there have been more frequent searches for spectro-photometric variability that would indicate non-uniform cloud cover (e.g. \citealt{ackerman01}) and weather-like features, such as those seen on Jupiter.
The majority of these early searches concentrated on L dwarfs, suggesting that variability could be due to holes in the clouds \citep{gelino02, ackerman01}. Surveys appear to suggest that between 40-70\%  of objects are variable \citet{bailer01,gelino02,clarke02}, although most of these surveys involve small numbers of objects and  the authors vary on what is considered at detection. The majority of these studies were performed in the $I$ band where the amplitude of variability is at the 1-2\% level \citep{clarke02, clarke08} on timescales of tens of minutes to weeks, and is in general not periodic. There has now been a shift towards using the near-IR for variability studies \citep{enoch03,clarke08, khandrika13, girardin13} where the frequency of variability is estimated to be $\sim$10-40\%. So far, however, high amplitude periodic variability ($>3$\%) has been limited to the L-T transition objects, while lower amplitude variability is detected in both early L and late T dwarfs.

The first T dwarf to be confirmed as variable was the T2.5 dwarf SIMP J013656.5+093347 \citep{artigau09} which was determined to be variable at the 50 mmag level in the $J$ band.  Using the lightcurves, a rotation period of 2.4 days was determined. However, perhaps more interestingly, the lightcurve evolves from night to night (Figure 2 of \citet{artigau09}), perhaps due to evolving features such as storms.  \citet{radigan12} studied a similar object, the T1.5 dwarf 2MASS2139, and again found evidence of an evolving light curve in the $J$, and $K_s$ wavebands, which after extensive modelling analysis they attributed to heterogeneous clouds with regions of higher opacity. In general these objects exhibit variable lightcurves, modulated as the object rotates, which evolve on a period of hours \citet{apai13}, days (e.g. \citealt {artigau09, radigan12} or even years \citet{metchev13}.

While the majority of T dwarfs that have been studied mostly lie at the L-T dwarf transition region, some late T dwarfs  ($>$T5) have been determined to be variable \citep{clarke08}. Initially, these atmospheres were thought to be relatively cloud-free, however recent work by \citet{morley12} suggests that sulphide clouds may persist in these atmospheres. \citet{buenzli12} studied one such object and determined that while sinusoidal variability was present, there was also a phase offset between different wavelengths. This phase shift is directly linked to the pressure probed at each of the observed wavelengths. The lower pressure regions cause the highest phase lag with respect to the highest pressure layers. This lag may be as large as half a rotation period.  \citet{buenzli12} suggest this longitudinal variability may be caused by changes in cloud opacities, a "stacked-cell" atmosphere as sen in Saturn(e.g. \citealt{fletcher11} or a heterogeneous deep cloud layer with horizontal variations in temperature.

One of the largest space based surveys to date was performed by \citet{buenzli14} who studied 22 brown dwarfs ranging from L5 to T6 with $HST$. Six of these objects are determined to be variable with another 5 marked as potentially variable. They were not sensitive to objects with long periods,  but still determine that the majority of brown dwarfs have patchy atmospheres, and that there is no spectral type dependence on the fraction of dwarfs that are variable.

\citet{heinze13} Heinze reported sinusoidal variability of the L3 dwarf DENIS-P J1058.7-1548 in the $J$ and [3.6] micron bands, but no variability in the [4.5] micron band. They suggested that the variability may again be due to inhomogenous cloud cover, where the thickest clouds have the lowest effective temperature, but there may also be an effect related to magnetic activity (starspots, chromospheric or  aurorae) due to a weak H$\alpha$ detection. This result is similar to the findings on the radio loud M8.5 dwarf TVLM513-46546 \citep{littlefair08}. TVLM513  shows $i'$ and $g'$ band variability in antiphase, initially suggesting the variability is due to dust clouds. However, more recent results show that the $g'$ and $i$ bands are no longer correlated. The $g'$ band variability has remained stable, but the $i'$ band lightcurve has evolved. However, the optical continuum variability is in phase with the H$\alpha$ flux, again suggesting some magnetic processes are also occurring \citep{metchev13}.

Luhman 16 is the third closest system to the sun at only 2pc \citep{luhman13} consisting of a L7.5 and T0.5 dwarf in a binary. \citet{gillon13} reported variability on a 4.87 hour period with strong night to night evolution which they attributed to a fast evolving atmosphere on the cooler T0.5 dwarf. The L7.5 dwarf is not found to be variable. \citet{burgasser14}  perfumed spectral monitoring of the system and confirmed the lack of variability in the L dwarf. They modelled the T dwarf using a two-spot model and inferred a cold covering fraction of $\sim$30-55\% varying by 15-30\% over a rotation period. This resulted in a difference of $\sim$200-400 K between the hot and cold regions.  \citet{burgasser14} interpreted the variations in temperature as changes in the covering fraction of a high cloud deck resulting in cloud holes which expose the deeper, hotter cloud layers. They also suggested the rapidly evolving atmosphere may produce winds as high as 1-3 kms$^{-1}$ which is consistent with  an advection timescale of 1-3 rotation periods.  The most in depth analysis of this system however, was produced by \citet{crossfield14} who used Doppler imaging techniques to produce a global surface map, mainly sensitive to CO,  of the T dwarf Luhman 16B. The map shows a large, dark mid-lattitude region, a brighter area on the opposite hemisphere located near the pole and mottling at equatorial latitudes (Figure 2 of \citealt{crossfield14}). The authors interpreted the map in one of two ways. Either the darker areas represent thicker clouds, obscuring the hotter, inner regions of the atmosphere, and the bright regions correspond to cloud holes providing a view of this warmer interior, or the map shows a combination of surface brightness and chemical abundance variations.  They predict that the high latitude bright spot could be similar to polar vortices seen in solar system giant planets, in which case it should be seen in future mapping of this object.  


Another class of brown dwarfs that show photometric variability are those in close ($<$10 hrs) detached binary systems with white dwarfs (WD0137-349, WD+L6-L8, P=116 min \citealt{maxted06, burleigh06}; GD1400, WD+L6, P=9.98hrs \citealt{farihi,  dobbie, burleigh11}; WD0837+185, WD+T8, P=4.2hrs \citealt{casewell12}; NLTT5306, WD+L4-L7, P=101.88 min \citealt{steele13}; CSS21055, WD+L, P=121.73 min \citealt{beuermann13}).
These systems are
likely tidally locked and as a result one side of the brown dwarf is continually heated by its much hotter white dwarf companion. Three of the five known systems show
variability in optical wavelengths at the 1\% level. One of these objects, WD0137-349 has been studied extensively at in the near-infrared \citep{casewell13}. The white dwarf in this system is 10 times hotter than the brown dwarf, resulting in a difference in brightness temperature of $\sim$500K. While the substellar objects in these systems are brown dwarfs, and not extrasolar planets, their atmospheres behave in a similar way, both absorbing the (mainly) ultraviolet
emissions from their host, and also reflecting the incident light. 


